The LSST Dark Energy Science Collaboration (DESC) Science Requirements Document

The Large Synoptic Survey Telescope (LSST) Dark Energy Science Collaboration (DESC) will use five cosmological probes: galaxy clusters, large scale structure, supernovae, strong lensing, and weak lensing. This Science Requirements Document (SRD) quantifies the expected dark energy constraining power of these probes individually and together, with conservative assumptions about analysis methodology and follow-up observational resources based on our current understanding and the expected evolution within the field in the coming years. We then define requirements on analysis pipelines that will enable us to achieve our goal of carrying out a dark energy analysis consistent with the Dark Energy Task Force definition of a Stage IV dark energy experiment. This is achieved through a forecasting process that incorporates the flowdown to detailed requirements on multiple sources of systematic uncertainty. Future versions of this document will include evolution in our software capabilities and analysis plans along with updates to the LSST survey strategy.

==> inc/commitID.tex <==
{\Large\bfseries Version~1.0.2}
% {\Large\bfseries Version~0.99.\href{COMMITURL}{\texttt{SHA}}} \\
% This is a current, intermediate version of the LSST DESC SRD \\
% which contains edits relative to
% % the formally released \href{\urlvonepointzero}{version v1.0}.
% \href{https://github.com/LSSTDESC/Requirements/releases/tag/v0.9}{version v0.9}.

\medskip
Date: September 6, 2021
% Branch: \href{BRANCHURL}{\texttt{BRANCH}} \\
% Most recent commit: \href{COMMITURL}{\texttt{SHA}} \\
% Date: DATE

